Optimization in Knowledge-Intensive Crowdsourcing

We present SmartCrowd, a framework for optimizing collaborative knowledge-intensive crowdsourcing. SmartCrowd distinguishes itself by accounting for human factors in the process of assigning tasks to workers. Human factors designate workers' expertise in different skills, their expected minimum wage, and their availability. In SmartCrowd, we formulate task assignment as an optimization problem, and rely on pre-indexing workers and maintaining the indexes adaptively, in such a way that the task assignment process gets optimized both qualitatively, and computation time-wise. We present rigorous theoretical analyses of the optimization problem and propose optimal and approximation algorithms. We finally perform extensive performance and quality experiments using real and synthetic data to demonstrate that adaptive indexing in SmartCrowd is necessary to achieve efficient high quality task assignment.

==> application.tex <==
\subsection{Motivating Applications}

==> submodular.tex <==
\section{Submodularity Proof}
\begin{theorem}
The value function $v_t$ in Section~\ref{obj} is submodular, when $Q_{t_m}=0$.
\end{theorem}

\begin{proof}
Consider an arbitrary function $f()$ that maps the subsets of a finite ground set $\mathcal{N}$ to non-negative real numbers. Our value function $v_t$ for task $t$ satisfies this form: it maps each subset of the workers $\mathcal{S}$ to a real number $v_t$ for a task $t$, denoting the value if that subset of workers are assigned to task $t$. 

The value function $v_t$ is a linear combination of two functions: skill and cost along with a set of constraints. For the purpose of illustration , we ignore the constant weights for now, as that does not impact the proof. A property of the skill function $f'() = \Sigma_{\forall m} q_{t_m}$ is as follows: for any $\mathcal{R} \subset \mathcal{S}$, and an element $k \in \mathcal{N} - \mathcal{S}$, adding $k$ to 
$\mathcal{S}$ will increase $f'()$ by no more than by adding $k$ to $\mathcal{R}$. Therefore,
\begin{equation}
f'(\mathcal{S} \cup k) -  f'(\mathcal{S}) \leq f'(\mathcal{R} \cup k) -  f'(\mathcal{R})
\end{equation}
For our problem, the above constraint actually satisfies the equality condition, because adding a worker to a task always increases $\Sigma_{\forall m} q_{t_m}$ by the amount of the skill of the worker, irrespective of whether it is added to $\mathcal{S}$ or $\mathcal{R}$. Therefore, $f'()$ is submodular.

Now, the cost function $f''() = (1-\frac{w_t}{W_t})$ also satisfies the following property: for any $\mathcal{R} \subset \mathcal{S}$, and an element $k \in \mathcal{N} - \mathcal{S}$, adding $k$ to $\mathcal{S}$ will increase $f''()$ by no more than by adding $k$ to $\mathcal{R}$. In fact, $f''()$ strictly decreases. Therefore, $f''()$ is also submodular and strictly decreasing. 

When $f'()$ and $f''()$ are combined linearly in $f()$ to obtain $v_t$, the following property also holds:
\begin{equation}
f(\mathcal{S} \cup k) -  f(\mathcal{S}) < f(\mathcal{R} \cup k) -  f(\mathcal{R})
\end{equation}
The reason is: the effect of $f'()$ is same on $f(\mathcal{S} \cup k) -  f(\mathcal{S})$ and on $f(\mathcal{R} \cup k) -  f(\mathcal{R}$. However, $f''()$ will decrease  in $f(\mathcal{S} \cup k) -  f(\mathcal{S})$ compared to that of in  $f(\mathcal{R} \cup k) -  f(\mathcal{R}$. Therefore,  the overall value function $v_t$ is also submodular.

The cost threshold: $w_t \leq W_t$ also satisfies submodularity, because  adding a new worker $k$ to $\mathcal{S}$ can make make $v_t=0$\footnote{\small if it surpasses the cost threshold} than adding $k$ to $\mathcal{R}$ (where  $\mathcal{R} \subset \mathcal{S}$), but the ``diminishing return'' property still holds: i.e.,
\begin{equation}
f(\mathcal{S} \cup k) -  f(\mathcal{S}) < f(\mathcal{R} \cup k) -  f(\mathcal{R})
\end{equation}
Hence the proof.
\end{proof}
